Efficient User-Centric Privacy-Friendly and Flexible Wearable Data Aggregation and Sharing

Wearable devices can offer services to individuals and the public. However, wearable data collected by cloud providers may pose privacy risks. To reduce these risks while maintaining full functionality, healthcare systems require solutions for privacy-friendly data processing and sharing that can accommodate three main use cases: (i) data owners requesting processing of their own data, and multiple data requesters requesting data processing of (ii) a single or (iii) multiple data owners. Existing work lacks data owner access control and does not efficiently support these cases, making them unsuitable for wearable devices. To address these limitations, we propose a novel, efficient, user-centric, privacy-friendly, and flexible data aggregation and sharing scheme, named SAMA. SAMA uses a multi-key partial homomorphic encryption scheme to allow flexibility in accommodating the aggregation of data originating from a single or multiple data owners while preserving privacy during the processing. It also uses ciphertext-policy attribute-based encryption scheme to support fine-grain sharing with multiple data requesters based on user-centric access control. Formal security analysis shows that SAMA supports data confidentiality and authorisation. SAMA has also been analysed in terms of computational and communication overheads. Our experimental results demonstrate that SAMA supports privacy-preserving flexible data aggregation more efficiently than the relevant state-of-the-art solutions.

==> References.tex <==

@article{sharma2018toward,
  title={Toward practical privacy-preserving analytics for IoT and cloud-based healthcare systems},
  author={Sharma, Sagar and Chen, Keke and Sheth, Amit},
  journal={IEEE Internet Computing},
  volume={22},
  number={2},
  pages={42--51},
  year={2018},
  publisher={IEEE}
}

@inproceedings{chen2022cloud,
  title={A Cloud-Assisted Data Processing Scheme for Smart Grid with Flexible Access Control},
  author={Chen, Shi and Wang, Jingjing and Yu, Zheng and Xu, Huan and Dong, Chenxi},
  booktitle={Proceedings of the 2022 5th International Conference on Algorithms, Computing and Artificial Intelligence},
  pages={1--6},
  year={2022}
}

@inproceedings{wang2023secure,
  title={Secure and Efficient Data Processing for Cloud Computing with Fine-Grained Access Control},
  author={Wang, Jingjing and Feng, Hao and Yu, Zheng and Liao, Rongtao and Chen, Shi and Liang, Ting},
  booktitle={International Symposium on Security and Privacy in Social Networks and Big Data},
  pages={187--202},
  year={2023},
  organization={Springer}
}
@article{lindell2017simulate,
  title={How to simulate it--a tutorial on the simulation proof technique},
  author={Lindell, Yehuda},
  journal={Tutorials on the Foundations of Cryptography: Dedicated to Oded Goldreich},
  pages={277--346},
  year={2017},
  publisher={Springer}
}
@inproceedings{wang2014tale,
  title={A tale of two clouds: Computing on data encrypted under multiple keys},
  author={Wang, Boyang and Li, Ming and Chow, Sherman and Li, Hui},
  booktitle={2014 IEEE Conference on Communications and Network Security},
  pages={337--345},
  year={2014}
}
@article{safavi2014conceptual,
  title={Conceptual privacy framework for health information on wearable device},
  author={Safavi, Seyedmostafa and Shukur, Zarina},
  journal={PLoS ONE},
  volume={9},
  number={12},
  pages={1--16},
  year={2014},
  publisher={Public Library of Science}
}


@inproceedings{datta2018survey,
  title={A Survey of Privacy Concerns in Wearable Devices},
  author={Datta, Prerit and Namin, Akbar Siami and Chatterjee, Moitrayee},
  booktitle={2018 IEEE International Conference on Big Data (Big Data)},
  pages={4549--4553},
  year={2018},
  organization={IEEE}
}

@article{bos2014private,
  title={Private predictive analysis on encrypted medical data},
  author={Bos, Joppe W and Lauter, Kristin and Naehrig, Michael},
  journal={Journal of biomedical informatics},
  volume={50},
  pages={234--243},
  year={2014},
  publisher={Elsevier}
}
@inproceedings{hassanalieragh2015health,
  title={Health monitoring and management using Internet-of-Things (IoT) sensing with cloud-based processing: Opportunities and challenges},
  author={Hassanalieragh, Moeen and Page, Alex and Soyata, Tolga and Sharma, Gaurav and Aktas, Mehmet and Mateos, Gonzalo and Kantarci, Burak and Andreescu, Silvana},
  booktitle={2015 IEEE International Conference on Services Computing},
  pages={285--292},
  year={2015},
  organization={IEEE}
}

@article{morris2013analysis,
  title={Analysis of partially and fully homomorphic encryption},
  author={Morris, Liam},
  journal={Rochester Institute of Technology},
  pages={1--5},
  year={2013}
}

@article{brakerski2014leveled,
  title={(Leveled) fully homomorphic encryption without bootstrapping},
  author={Brakerski, Zvika and Gentry, Craig and Vaikuntanathan, Vinod},
  journal={ACM Transaction on Computation Theory (TOCT)},
  volume={6},
  number={3},
  pages={13},
  year={2014},
  publisher={ACM}
}

@article{gentry2010computing,
  title={Computing arbitrary functions of encrypted data},
  author={Gentry, Craig},
  journal={Communications of the ACM},
  volume={53},
  number={3},
  pages={97--105},
  year={2010},
  publisher={ACM}
}
@article{liu2018hybrid,
  title={Hybrid privacy-preserving clinical decision support system in fog--cloud computing},
  author={Liu, Ximeng and Deng, Robert H and Yang, Yang and Tran, Hieu N and Zhong, Shangping},
  journal={Future Generation Computer Systems},
  volume={78},
  pages={825--837},
  year={2018},
  publisher={Elsevier}
}

@article{wang2013exploring,
  title={Exploring the feasibility of fully homomorphic encryption},
  author={Wang, Wei and Hu, Yin and Chen, Lianmu and Huang, Xinming and Sunar, Berk},
  journal={IEEE trans on Computers},
  volume={64},
  number={3},
  pages={698--706},
  year={2013},
  publisher={IEEE}
}

@inproceedings{cheon2013batch,
  title={Batch fully homomorphic encryption over the integers},
  author={Cheon, Jung Hee and Coron, Jean-S{\'e}bastien and Kim, Jinsu and Lee, Moon Sung and Lepoint, Tancrede and Tibouchi, Mehdi and Yun, Aaram},
  booktitle={Annual International Conference on the Theory and Applications of Cryptographic Techniques},
  pages={315--335},
  year={2013},
  organization={Springer}
}

@article{yan2014survey,
  title={A survey on trust management for Internet of Things},
  author={Yan, Zheng and Zhang, Peng and Vasilakos, Athanasios V},
  journal={Journal of network and computer applications},
  volume={42},
  pages={120--134},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{bogdanov2012deploying,
  title={Deploying secure multi-party computation for financial data analysis},
  author={Bogdanov, Dan and Talviste, Riivo and Willemson, Jan},
  booktitle={International Conference on Financial Cryptography and Data Security},
  pages={57--64},
  year={2012},
  organization={Springer}
}

@phdthesis{bogdanov2013sharemind,
  title={Sharemind: programmable secure computations with practical applications},
  author={Bogdanov, Dan},
  year={2013}
}

@article{kamm2015secure,
  title={Secure floating point arithmetic and private satellite collision analysis},
  author={Kamm, Liina and Willemson, Jan},
  journal={International Journal of Information Security},
  volume={14},
  number={6},
  pages={531--548},
  year={2015},
  publisher={Springer}
}

@article{peter2013efficiently,
  title={Efficiently outsourcing multiparty computation under multiple keys},
  author={Peter, Andreas and Tews, Erik and Katzenbeisser, Stefan},
  journal={IEEE Transaction on Information Forensics and Security},
  volume={8},
  number={12},
  pages={2046--2058},
  year={2013},
  publisher={IEEE}
}


@article{liu2016efficient,
  title={Efficient and privacy-preserving outsourced calculation of rational numbers},
  author={Liu, Ximeng and Choo, Kim-Kwang Raymond and Deng, Robert H and Lu, Rongxing and Weng, Jian},
  journal={IEEE Transaction on Dependable and Secure Computing},
  volume={15},
  number={1},
  pages={27--39},
  year={2016},
  publisher={IEEE}
}

@inproceedings{yan2015scheme,
  title={A scheme to manage encrypted data storage with deduplication in cloud},
  author={Yan, Zheng and Ding, Wenxiu and Zhu, Haiqi},
  booktitle={International Conference on Algorithms and Architectures for Parallel Processing},
  pages={547--561},
  year={2015},
  organization={Springer}
}
@article{othman2022privacy,
  title={Privacy-preserving aware data aggregation for IoT-based healthcare with green computing technologies},
  author={Othman, Soufiene Ben and Almalki, Faris A and Chakraborty, Chinmay and Sakli, Hedi},
  journal={Computers and Electrical Engineering},
  volume={101},
  pages={108025},
  year={2022},
  publisher={Elsevier}
}

@article{bhowmik2023eeppda,
  title={EEPPDA—Edge-enabled efficient privacy-preserving data aggregation in smart healthcare Internet of Things network},
  author={Bhowmik, Tanima and Banerjee, Indrajit},
  journal={International Journal of Network Management},
  pages={e2216},
  year={2023},
  publisher={Wiley Online Library}
}





@article{dong2011shared,
  title={Shared and searchable encrypted data for untrusted servers},
  author={Dong, Changyu and Russello, Giovanni and Dulay, Naranker},
  journal={Journal of Computer Security},
  volume={19},
  number={3},
  pages={367--397},
  year={2011},
  publisher={IOS Press}
}

@inproceedings{garrison2016practicality,
  title={On the practicality of cryptographically enforcing dynamic access control policies in the cloud},
  author={Garrison, William C and Shull, Adam and Myers, Steven and Lee, Adam J},
  booktitle={2016 IEEE Symposium on Security and Privacy (SP)},
  pages={819--838},
  year={2016},
  organization={IEEE}
}

@inproceedings{tianyi2011efficient,
  title={An efficient role based access control system for cloud computing},
  author={Tianyi, Zhu and Weidong, Liu and Jiaxing, Song},
  booktitle={2011 IEEE 11th International Conference on Computer and Information Technology},
  pages={97--102},
  year={2011},
  organization={IEEE}
}

@article{yan2015flexible,
  title={Flexible data access control based on trust and reputation in cloud computing},
  author={Yan, Zheng and Li, Xueyun and Wang, Mingjun and Vasilakos, Athanasios V},
  journal={IEEE Transaction on cloud Computing},
  volume={5},
  number={3},
  pages={485--498},
  year={2015},
  publisher={IEEE}
}

@article{yan2015controlling,
  title={Controlling cloud data access based on reputation},
  author={Yan, Zheng and Li, Xueyun and Kantola, Raimo},
  journal={Mobile Networks and Applications},
  volume={20},
  number={6},
  pages={828--839},
  year={2015},
  publisher={Springer}
}

@inproceedings{goyal2006attribute,
  title={Attribute-based encryption for fine-grained access control of encrypted data},
  author={Goyal, Vipul and Pandey, Omkant and Sahai, Amit and Waters, Brent},
  booktitle={Proceedings of the 13th ACM conference on Computer and communications security},
  pages={89--98},
  year={2006}
}

@article{xia2012internet,
  title={Internet of things},
  author={Xia, Feng and Yang, Laurence T and Wang, Lizhe and Vinel, Alexey},
  journal={International Journal of Communication Systems},
  volume={25},
  number={9},
  pages={1101},
  year={2012}
}

@article{li2012scalable,
  title={Scalable and secure sharing of personal health records in cloud computing using attribute-based encryption},
  author={Li, Ming and Yu, Shucheng and Zheng, Yao and Ren, Kui and Lou, Wenjing},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={24},
  number={1},
  pages={131--143},
  year={2012},
  publisher={IEEE}
}

@misc{siggelin2017seniors,
  title={Seniors Privacy Concerns in Health Technology Wearables: Regulations vs. User Concerns},
  author={Siggelin, Sofie},
  year={2017}
}

@inproceedings{yu2010achieving,
  title={Achieving secure, scalable, and fine-grained data access control in cloud computing},
  author={Yu, Shucheng and Wang, Cong and Ren, Kui and Lou, Wenjing},
  booktitle={2010 Proceedings IEEE INFOCOM},
  pages={1--9},
  year={2010},
  organization={Ieee}
}


@article{ruj2013decentralized,
  title={A decentralized security framework for data aggregation and access control in smart grids},
  author={Ruj, Sushmita and Nayak, Amiya},
  journal={IEEE Transaction on Smart Grid},
  volume={4},
  number={1},
  pages={196--205},
  year={2013},
  publisher={IEEE}
}

@inproceedings{rohloff2015end,
  title={An end-to-end security architecture to collect, process and share wearable medical device data},
  author={Rohloff, Kurt and Polyakov, Yuriy},
  booktitle={2015 17th International Conference on E-health Networking, Application \& Services (HealthCom)},
  pages={615--620},
  year={2015},
  organization={IEEE}
}

@article{fang2019fine,
  title={A Fine-Grained User-Divided Privacy-Preserving Access Control Protocol in Smart Watch},
  author={Fang, Liming and Li, Minghui and Zhou, Lu and Zhang, Hanyi and Ge, Chunpeng},
  journal={Sensors},
  volume={19},
  number={9},
  pages={2109},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{ding2017privacy1,
  title={Privacy-preserving data processing with flexible access control},
  author={Ding, Wenxiu and Yan, Zheng and Deng, Robert},
  journal={IEEE TDSC},
  year={2017},
  publisher={IEEE}
}
@ARTICLE{ding2017privacy,
  author={Ding, Wenxiu and Yan, Zheng and Deng, Robert},
  journal={IEEE Transactions on Dependable and Secure Computing}, 
  title={Privacy-Preserving Data Processing with Flexible Access Control}, 
  year={2020},
  volume={17},
  number={2},
  pages={363-376},
  doi={10.1109/TDSC.2017.2786247}}

@article{ding2017encrypted,
  title={Encrypted data processing with homomorphic re-encryption},
  author={Ding, Wenxiu and Yan, Zheng and Deng, Robert H},
  journal={Information Sciences},
  volume={409},
  pages={35--55},
  year={2017},
  publisher={Elsevier}
}

@article{alsharif2019epda,
  title={EPDA: Efficient and privacy-preserving data collection and access control scheme for multi-recipient AMI networks},
  author={Alsharif, Ahmad and Nabil, Mahmoud and Mahmoud, Mohamed MEA and Abdallah, Mohamed},
  journal={IEEE Access},
  volume={7},
  pages={27829--27845},
  year={2019},
  publisher={IEEE}
}

@article{sathya2018review,
  title={A review of homomorphic encryption libraries for secure computation},
  author={Sathya, Sai Sri and Vepakomma, Praneeth and Raskar, Ramesh and Ramachandra, Ranjan and Bhattacharya, Santanu},
  journal={arXiv preprint arXiv:1812.02428},
  year={2018}
}

@inproceedings{zickau2016applied,
  title={Applied attribute-based encryption schemes},
  author={Zickau, Sebastian and Thatmann, Dirk and Butyrtschik, Artjom and Denisow, Iwailo and K{\"u}pper, Axel},
  booktitle={19th International ICIN Conference-Innovations in Clouds, Internet and Networks},
  pages={88--95},
  year={2016}
}

@misc{ACUSInte73:online,
author = {Jason Healey, Neal Pollard, and Beau Woods},
title = {THE HEALTHCARE INTERNET OF THINGS REWARDS AND RISKS},
note = {\url{https://www.atlanticcouncil.org/wp-content/uploads/2015/03/ACUS\_Intel\_MedicalDevices.pdf}},
note = {(Accessed on 06/01/2020)}
}

@article{ching2016wearable,
 title={Wearable technology devices security and privacy vulnerability analysis},
  author={Ching, Ke Wan and Singh, Manmeet Mahinderjit},
  journal={International Journal of Network Security \& Its Applications},
  volume={8},
  number={3},
  pages={19--30},
  year={2016}
}
@incollection{motti2020wearable,
  title={Wearable Interaction},
  author={Motti, Vivian Genaro},
  booktitle={Wearable Interaction},
  publisher={Springer},
  pages={81--107},
  
  year={2020}

}

@misc{LINDDUNp35:online,
author = {},
title = {LINDDUN: a privacy threat analysis framework.pdf},
howpublished = {\url{https://people.cs.kuleuven.be/~kim.wuyts/LINDDUN/LINDDUN.pdf}},
month = {},
year = {},
note = {(Accessed on 06/20/2020)}
}

@misc{Advanced25:online,
author = {Jagannathan, Venkatesh},
title = {Threat Modelling Architecting & Designing with Security in Mind},
howpublished = {\url{https://owasp.org/www-pdf-archive/AdvancedThreatModeling.pdf}},
month = {},
year = {},
note = {(Accessed on 06/22/2020)}
}

@inproceedings{alshehri2012secure,
  title={Secure access for healthcare data in the cloud using ciphertext-policy attribute-based encryption},
  author={Alshehri, Suhair and Radziszowski, Stanislaw P and Raj, Rajendra K},
  booktitle={IEEE 28th international conference on data engineering workshops},
  pages={143--146},
  year={2012},
  organization={IEEE}
}


@article{COVID19W78:online,
  title={Real-time Alerting System for COVID-19 Using Wearable Data},
  author={Alavi, Arash and Bogu, Gireesh K and Wang, Meng and Rangan, Ekanath Srihari and Brooks, Andrew W and Wang, Qiwen and Higgs, Emily and Celli, Alessandra and Mishra, Tejaswini and Metwally, Ahmed A and others},
  journal={medRxiv},
  year={2021},
}

@article{sun2018private,
  title={Private machine learning classification based on fully homomorphic encryption},
  author={Sun, Xiaoqiang and Zhang, Peng and Liu, Joseph K and Yu, Jianping and Xie, Weixin},
  journal={IEEE Transaction on Emerging Topics in Computing},
  year={2018},
  publisher={IEEE}
}
@article{lagendijk2012encrypted,
  title={Encrypted signal processing for privacy protection: Conveying the utility of homomorphic encryption and multiparty computation},
  author={Lagendijk, Reginald L and Erkin, Zekeriya and Barni, Mauro},
  journal={IEEE Signal Processing Magazine},
  volume={30},
  number={1},
  pages={82--105},
  year={2012},
  publisher={IEEE}
}

@article{acar2018survey,
  title={A survey on homomorphic encryption schemes: Theory and implementation},
  author={Acar, Abbas and Aksu, Hidayet and Uluagac, A Selcuk and Conti, Mauro},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={4},
  pages={1--35},
  year={2018},
  publisher={ACM New York, NY, USA}
}
@inproceedings{belguith2016pabac,
  title={Pabac: a privacy preserving attribute based framework for fine grained access control in clouds},
  author={Belguith, Sana and Kaaniche, Nesrine and Jemai, Abderrazak and Laurent, Maryline and Attia, Rabah},
  year={2016}
}
@inproceedings{wang2016sieve,
  title={Sieve: Cryptographically enforced access control for user data in untrusted clouds},
  author={Wang, Frank and Mickens, James and Zeldovich, Nickolai and Vaikuntanathan, Vinod},
  booktitle={USENIX Symposium on Networked Systems Design and Implementation},
  pages={611--626},
  year={2016}
}
@article{ding2020extended,
  title={An Extended Framework of Privacy-Preserving Computation With Flexible Access Control},
  author={Ding, Wenxiu and Hu, Rui and Yan, Zheng and Qian, Xinren and Deng, Robert H and Yang, Laurence T and Dong, Mianxiong},
  journal={IEEE Transactions on Network and Service Management},
  volume={17},
  number={2},
  pages={918--930},
  year={2020},
  publisher={IEEE}
}
@article{tang2019efficient,
  title={Efficient and privacy-preserving fog-assisted health data sharing scheme},
  author={Tang, Wenjuan and Ren, Ju and Zhang, Kuan and Zhang, Deyu and Zhang, Yaoxue and Shen, Xuemin},
  journal={ACM Transactions on Intelligent Systems and Technology},
  volume={10},
  number={6},
  pages={1--23},
  year={2019},
  publisher={ACM New York, NY, USA}
}
@article{pang2021privacy,
  title={Privacy-Preserving Association Rule Mining Using Homomorphic Encryption in a Multikey Environment},
  author={Pang, Hongping and Wang, Baocang},
  journal={IEEE Systems Journal},
  volume={15},
  number={2},
  pages={3131--3141},
  year={2021}
}
@article{aloufi2020computing,
  title={Computing blindfolded on data homomorphically encrypted under multiple keys: An extended survey},
  author={Aloufi, Asma and Hu, Peizhao and Song, Yongsoo and Lauter, Kristin},
  journal={arXiv preprint arXiv:2007.09270},
  year={2020}
}
@article{islam2020wearable,
  title={Wearable technology to assist the patients infected with coronavirus (COVID-19)},
  author={Islam, Md Milon and Mahmud, Saifuddin and Muhammad, LJ and Islam, Md Rabiul and Nooruddin, Sheikh and Ayon, Safial Islam},
  journal={SN Computer Science},
  volume={1},
  number={6},
  pages={1--9},
  year={2020},
  publisher={Springer}
}
@inproceedings{shafagh2017secure,
  title={Secure sharing of partially homomorphic encrypted iot data},
  author={Shafagh, Hossein and Hithnawi, Anwar and Burkhalter, Lukas and Fischli, Pascal and Duquennoy, Simon},
  booktitle={ Int. Conf. on Embedded Network Sensor Systems},
  pages={1--14},
  publisher={ACM},
  year={2017}
}
@inproceedings{paillier1999public,
  title={Public-key cryptosystems based on composite degree residuosity classes},
  author={Paillier, Pascal},
  booktitle={International conference on the theory and applications of cryptographic techniques},
  pages={223--238},
  year={1999},
  organization={Springer}
}
@inproceedings{waters2011ciphertext,
  title={Ciphertext-policy attribute-based encryption: An expressive, efficient, and provably secure realization},
  author={Waters, Brent},
  booktitle={International Workshop on Public Key Cryptography},
  pages={53--70},
  year={2011},
  organization={Springer}
}
@article{domingo2019privacy,
  title={Privacy-preserving cloud computing on sensitive data: A survey of methods, products and challenges},
  author={Domingo-Ferrer, Josep and Farr{\`a}s, Oriol and Ribes-Gonz{\'a}lez, Jordi and S{\'a}nchez, David},
  journal={Computer Communications},
  volume={140},
  pages={38--60},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{bethencourt2007ciphertext,
  title={Ciphertext-policy attribute-based encryption},
  author={Bethencourt, John and Sahai, Amit and Waters, Brent},
  booktitle={2007 IEEE symposium on security and privacy},
  pages={321--334},
  year={2007},
}

@article{wang2012java,
  title={Java Realization for Ciphertext-Policy Attribute-Based Encryption},
  author={Wang, Junwei},
   url ={\url{https://github.com/junwei-wang/cpabe/}},
  year={2012}
}

@article{zhou2015security,
  title={Security and privacy in cloud-assisted wireless wearable communications: challenges, solutions, and future directions},
  author={Zhou, Jun and Cao, Zhenfu and Dong, Xiaolei and Lin, Xiaodong},
  journal={IEEE Wireless Communications},
  volume={22},
  number={2},
  pages={136--144},
  year={2015},
  publisher={IEEE}
}


@article{xiao2012efficient,
  title={An efficient homomorphic encryption protocol for multi-user systems},
  author={Xiao, Liangliang and Bastani, Osbert and Yen, I-Ling},
  journal={Cryptology ePrint Archive},
  year={2012}
}



@article{liu2019secure,
  title={Secure IoT data outsourcing with aggregate statistics and fine-grained access control},
  author={Liu, Ling and Wang, He and Zhang, Yuqing},
  journal={IEEE Access},
  volume={8},
  pages={95057--95067},
  year={2019},
  publisher={IEEE}
}

@article{feng2018privacy,
  title={Privacy-preserving tensor decomposition over encrypted data in a federated cloud environment},
  author={Feng, Jun and Yang, Laurence T and Zhu, Qing and Choo, Kim-Kwang Raymond},
  journal={IEEE Transaction on Dependable and Secure Computing},
  volume={17},
  number={4},
  pages={857--868},
  year={2018},
  publisher={IEEE}
}

@article{wu2018verifiable,
  title={Verifiable public key encryption with keyword search based on homomorphic encryption in multi-user setting},
  author={Wu, DN and Gan, QQ and Wang, XM},
  journal={IEEE Access},
  volume={6},
  pages={42445--42453},
  year={2018},
  publisher={IEEE}
}

@article{blatt2020secure,
  title={Secure large-scale genome-wide association studies using homomorphic encryption},
  author={Blatt, Marcelo and Gusev, Alexander and Polyakov, Yuriy and Goldwasser, Shafi},
  journal={NAS},
  volume={117},
  number={21},
  pages={11608--11613},
  year={2020},
  publisher={National Acad Sciences}
}
@article{mustafa2015dep2sa,
  title={DEP2SA: A decentralized efficient privacy-preserving and selective aggregation scheme in AMI},
  author={Mustafa, Mustafa A and Zhang, Ning and Kalogridis, Georgios and Fan, Zhong},
  journal={IEEE Access},
  volume={3},
  pages={2828--2846},
  year={2015},
  publisher={IEEE}
}
@article{zhang2022distributed,
  title={A distributed privacy-preserving data aggregation scheme for smart grid with fine-grained access control},
  author={Zhang, Wenzheng and Liu, Shiyun and Xia, Zhe},
  journal={Journal of Information Security and Applications},
  volume={66},
  year={2022},
  publisher={Elsevier}
}
@article{li2022lightweight,
  title={Lightweight and Fine-Grained Privacy-Preserving Data Aggregation Scheme in Edge Computing},
  author={Li, Hongyang and Cheng, Qingfeng and Li, Xinghua and Ma, Siqi and Ma, Jianfeng},
  journal={IEEE Systems Journal},
  volume={16},
  number={2},
  pages={1832--1841},
  year={2022}
}
@article{wang2023ciphertext,
  title={Ciphertext-policy attribute-based encryption supporting policy-hiding and cloud auditing in smart health},
  author={Wang, Huiyong and Liang, Jialing and Ding, Yong and Tang, Shijie and Wang, Yujue},
  journal={Computer Standards \& Interfaces},
  volume={84},
  pages={103696},
  year={2023},
  publisher={Elsevier}
}
@article{aloufi2019blindfolded,
  title={Blindfolded evaluation of random forests with multi-key homomorphic encryption},
  author={Aloufi, Asma and Hu, Peizhao and Wong, Harry WH and Chow, Sherman SM},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={18},
  number={4},
  pages={1821--1835},
  year={2019},
  publisher={IEEE}
}

@inproceedings{chen2021non,
  title={Non-interactive Privacy-Preserving Na{\"\i}ve Bayes Classifier Using Homomorphic Encryption},
  author={Chen, Jingwei and Feng, Yong and Liu, Yang and Wu, Wenyuan and Yang, Guanci},
  booktitle={International Conference on Security and Privacy in New Computing Environments},
  pages={192--203},
  year={2021},
  organization={Springer}
}

@inproceedings{lopez2012fly,
  title={On-the-fly multiparty computation on the cloud via multikey fully homomorphic encryption},
  author={L{\'o}pez-Alt, Adriana and Tromer, Eran and Vaikuntanathan, Vinod},
  booktitle={ACM symposium on Theory of computing},
  pages={1219--1234},
  year={2012}
}

@article{ding2019survey,
  title={A survey on data fusion in internet of things: Towards secure and privacy-preserving fusion},
  author={Ding, Wenxiu and Jing, Xuyang and Yan, Zheng and Yang, Laurence T},
  journal={Information Fusion},
  volume={51},
  pages={129--144},
  year={2019},
  publisher={Elsevier}
}

@article{liu2019survey,
  title={A survey on secure data analytics in edge computing},
  author={Liu, Dan and Yan, Zheng and Ding, Wenxiu and Atiquzzaman, Mohammed},
  journal={IEEE Internet of Things Journal},
  volume={6},
  number={3},
  pages={4946--4967},
  year={2019},
  publisher={IEEE}
}
@article{zhang2021privacy,
  title={Privacy-preserving multikey computing framework for encrypted data in the cloud},
  author={Zhang, Jun and Jiang, Zoe L and Li, Ping and Yiu, Siu Ming},
  journal={Information Sciences},
  volume={575},
  pages={217--230},
  year={2021},
  publisher={Elsevier}
}
@article{ara2017secure,
  title={A secure privacy-preserving data aggregation scheme based on bilinear ElGamal cryptosystem for remote health monitoring systems},
  author={Ara, Anees and Al-Rodhaan, Mznah and Tian, Yuan and Al-Dhelaan, Abdullah},
  journal={IEEE Access},
  volume={5},
  pages={12601--12617},
  year={2017},
  publisher={IEEE}
}
@article{wang2019achieve,
  title={Achieve privacy-preserving priority classification on patient health data in remote eHealthcare system},
  author={Wang, Guoming and Lu, Rongxing and Guan, Yong Liang},
  journal={IEEE Access},
  volume={7},
  pages={33565--33576},
  year={2019},
  publisher={IEEE}
}

@article{erkin2012generating,
  title={Generating private recommendations efficiently using homomorphic encryption and data packing},
  author={Erkin, Zekeriya and Veugen, Thijs and Toft, Tomas and Lagendijk, Reginald L},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={7},
  number={3},
  pages={1053--1066},
  year={2012},
  publisher={IEEE}
}
@article{zhou2015ppdm,
  title={{PPDM:} Privacy-preserving protocol for dynamic medical text mining and image feature extraction from secure data aggregation in cloud-assisted e-healthcare systems},
  author={Zhou, Jun and Cao, Zhenfu and Dong, Xiaolei and Lin, Xiaodong},
  journal={IEEE J. of Selected Topics in Signal Processing},
  volume={9},
  number={7},
  pages={1332--1344},
  year={2015}
}

@inproceedings{zhang2015foresee,
  title={Foresee: Fully outsourced secure genome study based on homomorphic encryption},
  author={Zhang, Yuchen and Dai, Wenrui and Jiang, Xiaoqian and Xiong, Hongkai and Wang, Shuang},
  booktitle={BMC medical informatics and decision making},
  volume={15},
  number={5},
  pages={1--11},
  year={2015},
  organization={Springer}
}


@article{aloufi2020computing,
  title={Computing blindfolded on data homomorphically encrypted under multiple keys: An extended survey},
  author={Aloufi, Asma and Hu, Peizhao and Song, Yongsoo and Lauter, Kristin},
  journal={arXiv preprint arXiv:2007.09270},
  year={2020}
}

@inproceedings{ISCC:DecIov11,
    author    = {Angelo {De Caro} and Vincenzo Iovino},
    title     = {jPBC: Java pairing based cryptography},
    year      = {2011},
    pages     = {850-855},
    booktitle = {Symposium on Computers and Communications},
    publisher = {IEEE},
    url       = {\url{http://gas.dia.unisa.it/projects/jpbc/}},
}

@misc{Aguideto89:online,
author = {},
title = {A guide to GDPR data privacy requirements -- {GDPR.EU}},
howpublished = {\url{https://gdpr.eu/data-privacy}},
month = {},
year = {},
note = {(Accessed on 02/03/2022)}
}

@misc{EURLex3254:online,
author = {},
title = {EUR-Lex - 32016R0679 - EN - EUR-Lex},
howpublished = {\url{https://eur-lex.europa.eu/eli/reg/2016/679/oj}},
month = {},
year = {},
note = {(Accessed on 02/03/2022)}
}

@misc{REGULATI80:online,
author = {},
title = {Regulation ({EU}) 2016 - General Data Protection Regulation},
URL = {\url{https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=CELEX:32016R0679}},
month = {},
year = {},
note = {(Accessed on 02/03/2022)}
}

@article{act1996health,
  title={Health insurance portability and accountability act of 1996},
  author={Act, Accountability},
  journal={Public Law},
  volume={104},
  pages={191},
  year={1996}
}
@inproceedings{sahai2005fuzzy,
  title={Fuzzy identity-based encryption},
  author={Sahai, Amit and Waters, Brent},
  booktitle={Int.l Conf. on the TACT},
  pages={457--473},
  year={2005},
  organization={Springer}
}

@inproceedings{gentry2009fully,
  title={Fully homomorphic encryption using ideal lattices},
  author={Gentry, Craig},
  booktitle={Proceedings of the forty-first annual ACM symposium on Theory of computing},
  pages={169--178},
  year={2009}
} 

@inproceedings{narayan2010privacy,
  title={Privacy preserving EHR system using attribute-based infrastructure},
  author={Narayan, Shivaramakrishnan and Gagn{\'e}, Martin and Safavi-Naini, Reihaneh},
  booktitle={Proceedings of the 2nd ACM Cloud Computing Security Workshop},
  pages={47--52},
  year={2010}
}
@article{liu2015secure,
  title={Secure sharing of personal health records in cloud computing: Ciphertext-policy attribute-based signcryption},
  author={Liu, Jianghua and Huang, Xinyi and Liu, Joseph K},
  journal={Future Generation Computer Systems},
  volume={52},
  pages={67--76},
  year={2015},
  publisher={Elsevier}
}


@article{aloufi2021computing,
  title={Computing blindfolded on data homomorphically encrypted under multiple keys: A survey},
  author={Aloufi, Asma and Hu, Peizhao and Song, Yongsoo and Lauter, Kristin},
  journal={ACM Computing Surveys},
  volume={54},
  number={9},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY}
}
@inproceedings{shafagh2020droplet,
  title={Droplet: Decentralized authorization and access control for encrypted data streams},
  author={Shafagh, Hossein and Burkhalter, Lukas and Ratnasamy, Sylvia and Hithnawi, Anwar},
  booktitle={USENIX Security Symposium},
  pages={2469--2486},
  year={2020}
}

@article{li2021efficient,
  title={An efficient ciphertext-policy weighted attribute-based encryption for the internet of health things},
  author={Li, Hang and Yu, Keping and Liu, Bin and Feng, Chaosheng and Qin, Zhiguang and Srivastava, Gautam},
  journal={IEEE Journal of Biomedical and Health Informatics},
  year={2021},
  publisher={IEEE}
}
}

@article{zhong2021efficient,
  title={An efficient and outsourcing-supported attribute-based access control scheme for edge-enabled smart healthcare},
  author={Zhong, Hong and Zhou, Yiyuan and Zhang, Qingyang and Xu, Yan and Cui, Jie},
  journal={Future Generation Computer Systems},
  volume={115},
  pages={486--496},
  year={2021},
  publisher={Elsevier}
}



}

==> includes/khlood_261223.tex <==
\renewcommand{\rmdefault}{phv}

\definecolor{colorOne}{rgb}{0.1,0.1,0.1}
\definecolor{colorOneFill}{rgb}{0.6,0.6,0.6}

\definecolor{colorTwoFill}{rgb}{0.8,0.8,0.8}

\definecolor{colorThree}{rgb}{0.95,0.66,0.41}
\definecolor{colorThreeFill}{rgb}{1.0,0.86,0.6}

\definecolor{colorFour}{rgb}{0.54,0.6,0.8}
\definecolor{colorFourFill}{rgb}{0.57,0.73,0.88}

\definecolor{colorFive}{rgb}{0.53,0.6,0.84}
\definecolor{colorFiveFill}{rgb}{0.8,0.8,1}

\definecolor{colorSix}{rgb}{0.25,0.25,0.25}

%%% boxs functions
\def\boxr#1#2#3#4#5#6#7#8{
	\begin{tikzpicture}[xscale=#6, yscale=#7]
		\filldraw[line width=0.4mm, color= #4, rounded corners=10, fill=#5, drop shadow={shadow xshift=0.4ex, shadow yshift=-0.4ex, opacity=0.3}] (-3.1,-1.25) rectangle (3.1,1.25);
		\node at (0,#8)[]{
			\begin{tikzpicture}[scale=0.65]
				\node at (0,1)[color=black, scale=1.05]{\Large{\textbf{#1}}};
				\node at (0,0)[color=black, scale=1.05]{\Large{\textbf{#2}}};
				\node at (0,-1)[color=black, scale=1.05]{\Large{\textbf{#3}}};
			\end{tikzpicture}
		};
	\end{tikzpicture}
}

\def\boxrshade#1#2#3#4#5#6#7#8{
	\begin{tikzpicture}[xscale=#6, yscale=#7]
		\shade[bottom color=#5, top color= #5!10, fill=#5, rounded corners=10, drop shadow={shadow xshift=0.4ex, shadow yshift=-0.4ex, opacity=0.3}] (-3.1,-1.25) rectangle (3.1,1.25);
		\draw[line width=0.4mm, color= #4, rounded corners=10] (-3.1,-1.25) rectangle (3.1,1.25);
		\node at (0,#8)[]{
			\begin{tikzpicture}[scale=0.65]
				\node at (0,1)[color=black, scale=1.05]{\Large{\textbf{#1}}};
				\node at (0,0)[color=black, scale=1.05]{\Large{\textbf{#2}}};
				\node at (0,-1)[color=black, scale=1.05]{\Large{\textbf{#3}}};
			\end{tikzpicture}
		};
	\end{tikzpicture}
}


\def\DiagramDecember#1{\begin{tikzpicture}
		\node at (0,0)[scale=#1]{
			\begin{tikzpicture}
				\def\x{0.8}
				\def\y{1}
				\draw[line width=0.8mm, color=colorSix] 
				(0,1.75)node[]{\boxrshade{}{Privacy Enhancing}{Techniques (PETs)}{colorOne}{colorOneFill}{1}{0.9}{0.25}} -- 
				(0,0) -- (-11+\y,0) (0,0) -- (11-\x,0) (-11+\y,0) -- 
				(-11+\y,-3.25)node[midway]{\boxrshade{}{Data Sharing}{}{colorOne}{colorTwoFill}{0.8}{0.9}{0}}
				(-16.3+\y,-5)node[]{\boxrshade{Role-based}{Access Control}{(RBAC)}{colorThree}{colorThreeFill}{0.8}{1}{-0.1}}
				-- (-16.3+\y,-3.25) -- (-11+\y,-3.25) -- 
				(-11+\y,-5)node[]{\boxrshade{Proxy Re-}{encryption (PRE)}{}{colorThree}{colorThreeFill}{0.8}{1}{-0.2}}
				(-11+\y,-3.25) -- (-5.7+\y,-3.25) --
				(-5.7+\y,-5)node[]{\boxrshade{Attribute-based}{Encyption (ABE)}{}{colorThree}{colorThreeFill}{0.8}{1}{-0.2}}
				-- (-7.7+\y,-5) -- (-7.7+\y,-12) -- 
				(-3.45+\y,-12)node[]{\boxr{Ciphertext-policy Attribute-}{based Encryption (CP-ABE)}{}{colorFour}{colorFourFill}{1.25}{1}{-0.2}}
				-- (-4.7+\y,-12) (-7.7+\y,-8.5) --
				(-3.45+\y,-8.5)node[]{\boxr{Key-policy Attribute-based}{Encryption (KP-ABE)}{}{colorFour}{colorFourFill}{1.2}{1}{-0.2}}
				--(-4.7+\y,-9) (11-\x,0) -- %positif
				(11-\x,-3.25)node[midway]{\boxrshade{}{Data Processing}{}{colorOne}{colorTwoFill}{0.8}{0.9}{0}}
				(8.3-\x,-3.25) -- (13.7-\x,-3.25) --
				(13.7-\x,-5)node[]{\boxrshade{Secure Multi-Party}{Computation}{(MPC)}{colorThree}{colorThreeFill}{0.8}{1}{0}}
				(8.3-\x,-3.25) -- 
				(8.3-\x,-6.75)node[midway]{\boxrshade{Homomorphic}{Encyption (HE)}{}{colorThree}{colorThreeFill}{0.8}{1}{-0.2}}
				(5.3-\x,-6.75) -- (11.3-\x,-6.75)
				(5.3-\x,-6.75) -- 
				(5.3-\x,-8.5)node[]{\boxrshade{HE-based}{Operations}{}{colorFive}{colorFourFill}{0.8}{1}{-0.2}}
				-- (3.3-\x,-8.5) -- (3.3-\x,-18.2)
				(3.3-\x,-11.8) -- 
				(6.3-\x,-11.8) node[]{\boxr{Partially}{Homomorphic}{Encryption (PHE)}{colorFour}{colorFourFill}{0.85}{1}{0}}
				(3.3-\x,-15) -- 
				(6.3-\x,-15) node[]{\boxr{Somewhat}{Homomorphic}{Encryption (SWHE)}{colorFour}{colorFourFill}{0.85}{1}{0}}
				(3.3-\x,-18.2) -- 
				(6.3-\x,-18.2) node[]{\boxr{Fully}{Homomorphic}{Encryption (FHE)}{colorFour}{colorFourFill}{0.85}{1}{0}}
				(11.3-\x,-6.75) -- 
				(11.3-\x,-8.65)node[]{\boxrshade{HE-based Keys}{}{}{colorFive}{colorFourFill}{0.8}{1}{-0.55}}
				(11.3-\x,-8.5) -- (9.3-\x,-8.5) -- (9.3-\x,-15)
				(9.3-\x,-11.8) -- 
				(12.3-\x,-11.8) node[]{\boxr{Symmetric}{(Single-key)}{HE}{colorFour}{colorFourFill}{0.85}{1}{0}}
				(9.3-\x,-15) -- 
				(12.3-\x,-15) node[]{\boxr{Asymmetric}{(Multiple-keys)}{HE}{colorFour}{colorFourFill}{0.85}{1}{0}}
				;
        \end{tikzpicture}};
\end{tikzpicture}}

%end of defining function
